Identification of 1RXS J165424.6-433758 as a polar cataclysmic variable

We present the results of our X-ray, ultraviolet, and optical follow-up campaigns of 1RXS J165424.6-433758, an X-ray source detected with the \textit{Swift} Deep Galactic Plane Survey (DGPS). The source X-ray spectrum (\textit{Swift} and \textit{NuSTAR}) is described by thermal bremsstrahlung radiation with a temperature of $kT=10.1\pm1.2$ keV, yielding an X-ray ($0.3-10$ keV) luminosity $L_X=(6.5\pm0.8)\times10^{31}$ erg s$^{-1}$ at a \textit{Gaia} distance of 460 pc. Spectroscopy with the Southern African Large Telescope (SALT) revealed a flat continuum dominated by emission features, demonstrating an inverse Balmer decrement, the $\lambda4640$ Bowen blend, almost a dozen HeI lines, and HeII $\lambda4541$, $\lambda4686$ and $\lambda 5411$. Our high-speed photometry demonstrates a preponderance of flickering and flaring episodes, and revealed the orbital period of the system, $P_\textrm{orb}=2.87$ hr, which fell well within the cataclysmic variable (CV) period gap between $2-3$ hr. These features classify 1RXS J165424.6-433758 as a nearby polar magnetic CV.

==> old_table.tex <==
\begin{table*}
    \centering
    \caption{Results of our X-ray spectral fitting when including a partially covered absorber (\texttt{pcfabs}). \brendan{re-do these fits with pcfabs} \textcolor{red}{We can ignore this, Koji said it is ok.}
    }
    \label{tab: spectral_tableJ1654pcf}
    \begin{tabular}{lcccccc}
    \hline
    \hline
    &  & \multicolumn{4}{c}{\textbf{Models}} \\
    \cmidrule(lr){3-6}
    \textbf{Parameter} & \textbf{Units} &  \textbf{\texttt{pow}} & \textbf{\texttt{bremss}}  & \textbf{\texttt{mkcflow}} & \textbf{\texttt{ipolar}} \\
    \hline
    \multicolumn{6}{c}{\textbf{High-state}}\\
    \hline
    $N_H$ & $10^{22}$ cm$^{-2}$ & $0.49\pm0.07$ & $0.24\pm0.05$ & $0.35\pm0.05$ & \textcolor{red}{XX} \\
    $N_{H,pc}$ & $10^{22}$ cm$^{-2}$ & \textcolor{red}{XX} & \textcolor{red}{XX} &\textcolor{red}{XX} &\textcolor{red}{XX} \\
    $C_{pc}^a$ & -- & \textcolor{red}{XX} & \textcolor{red}{XX} &\textcolor{red}{XX} &\textcolor{red}{XX} \\
      $\Gamma$  & --& $2.02\pm0.07$ & -- & -- & -- \\
      $N_\texttt{pow}$  & $10^{-4}$ ph cm$^{-2}$ s$^{-1}$ & $8.1\pm1.3$ & -- &  -- & -- \\
     $kT$ & keV & --& $10.1\pm1.2$ & -- & -- \\
     $N_\texttt{bremss}$ & $10^{-4}$ &-- & $5.4\pm0.4$ & --& --\\
     $T_\textrm{high}$ & keV &-- & --& $21\pm3$ & --\\ 
     $A^b$ & -- & --&-- &  $0.8\pm0.3$& -- \\
      $N_\texttt{mkcflow}$ & $10^{-12} M_\odot$ yr$^{-1}$ &-- &-- & $20\pm4 $ & -- \\
    $M_\textrm{WD}$ & $M_\odot$ &-- &-- &-- & \\
    $R_m/R_\textrm{WD}$ & -- &-- &-- &-- & \\
    $N_\texttt{ipolar}$ & -- &-- &-- &-- & \\
    $C_\textrm{FPMA}$ & -- & 1.0 & 1.0 & 1.0& 1.0 \\
    $C_\textrm{FPMB}$ & -- &$0.94\pm0.07$ &$0.94\pm0.07$ & $0.94\pm0.07$& \\
    $C_\textrm{XRT}$ &-- & $0.63\pm0.07$ & $0.76\pm0.07$ &  $0.72\pm0.08$& \\
      Cstat &-- & 298/313 & 268/313  & 266/312 & \\
        \hline
    \multicolumn{6}{c}{\textbf{Low-state}}\\
    \hline
    $N_H$ & $10^{22}$ cm$^{-2}$ & $(8\pm5)\times10^{-2}$ & $(5\pm3)\times10^{-2}$ & -- & -- \\
    $N_{H,pc}$ & $10^{22}$ cm$^{-2}$ & -- & -- &-- &-- \\
    $C_{pc}^a$ & -- & -- & -- &-- & -- \\
      $\Gamma$  &-- & $1.6\pm0.2$ & -- & -- & -- \\
      $N_\texttt{pow}$  & $10^{-4}$ ph cm$^{-2}$ s$^{-1}$ & $0.12\pm0.02$ & --&  -- & --\\
          $kT$ & keV &-- & $8^{+9}_{-3}$ & --& --\\
     $N_\texttt{bremss}$ & $10^{-4}$ &-- & $0.15\pm0.02$ & --& --\\
      $T_\textrm{high}$ & keV &-- & --& -- & --\\ 
     $A^a$ & -- & --&-- & --& --\\
      $N_\texttt{mkcflow}$ & $10^{-12} M_\odot$ yr$^{-1}$ &-- &-- & -- & --\\
          $M_\textrm{WD}$ & $M_\odot$ &-- &-- &-- & --\\
    $R_m/R_\textrm{WD}$ & -- &-- &-- &-- & -- \\
    $N_\texttt{ipolar}$ & -- &-- &-- &-- & -- \\
    $C_\textrm{PN}$ & -- & 1.0 & 1.0 & --& --\\
    $C_\textrm{MOS1}$ &-- & $0.84\pm0.18$ & $0.82\pm0.16$ &-- & --\\
    $C_\textrm{MOS2}$ &-- & $1.05\pm0.20$ & $1.04\pm0.19$ &  -- & --\\
     Cstat/dof &-- & 816/824 & 816/824 & -- & --\\
   \hline
   \hline
   \end{tabular}
       \begin{flushleft}
     %\quad 
     \footnotesize{
     $^a$ Partial covering fraction. \\
     $^b$ Abundance relative to solar in the \texttt{mkcflow} model.\\
     }
\end{flushleft}
\end{table*}
